Collective Communication Patterns Using Time-Reversal Terahertz Links at the Chip Scale

Wireless communications in the terahertz band have been recently proposed as complement to conventional wired interconnects within computing packages. Such environments are typically highly reverberant, hence showing long channel impulse responses and severely limiting the achievable rates. Fortunately, this communications scenario is static and can be pre-characterized, which opens the door to techniques such as time reversal. Time reversal acts a spatial matched filter and has a spatiotemporal focusing effect, which allows not only to increase the achievable symbol rates, but also to create multiple spatial channels. In this paper, the multi-user capability of time reversal is explored in the context of wireless communications in the terahertz band within a computing package. Full-wave simulations are carried out to validate the approach, whereas modulation streams are simulated to evaluate the error rate as a function of the transmitted power, symbol rate, and number of simultaneous transmissions.

==> 1-intro.tex <==
%\hl{Expanded version of the abstract. Mention that reverberant environments create interferences in time and space, limiting speed and the creation of multiple spatial channels. TR can fix both. In this paper, we mainly explore the spatial consequences of TR.} 
Terahertz communications open the door to a wealth of opportunities in 6G networks and beyond due to not only the much-sought increase in bandwidth, but also the miniaturized size of antennas and transceivers operating in this band \cite{lemic2021survey}. Thanks to such miniaturization, new applications arise as wireless communications can be taken to unprecedented locations such as inside the human body \cite{saeed2021body,elayan2017terahertz} or within computing packages both in the classical \cite{chen2019channel, fu2020modeling, Yi2021} and quantum computing domains \cite{wang202334, alarcon2023scalable}.

Being considerably different than traditional wireless communication scenarios, novel applications often pose new challenges in the form of tight resource constraints (e.g. energy from harvesting sources), unfavorable channel conditions (e.g. enclosed and reverberant cavities), or performance requirements (e.g. ultra-low latency deadlines). Fortunately, these new environments may also offer some optimization opportunities that are typically not exploitable in conventional scenarios. In any case, these aspects force designers to rethink the entire protocol stack \cite{jornet2014femtosecond, franques2021fuzzy, tsioliaridou2017packet} and adapt it to the specific constraints and opportunities of these new and often extreme environments.

Among the new avenues to explore, this paper focuses on the application of wireless communications in the terahertz band (0.1-10 THz) within computing packages \cite{Sujay2012, Laha2015}. Such an idea is motivated by the recent emergence of massively parallel and heterogeneous computer architectures whose bottleneck generally lies in the intra-/inter-chip communications. In this context, communication has been traditionally served via on-chip networks formed by integrated routers linked with on-chip and chip-to-chip wired links, with simple topologies, routing and flow control mechanisms \cite{bertozzi2015fast}. However, as architectures scaled to handle massive parallelism and heterogeneity, these topologies suffered from multi-hop latency and energy efficiency issues, especially for collective communication patterns and when moving from chip to chip \cite{Karkar2016, Shamim2017}. 
%Over the past few decades, the increment of user needs has initiated the pathway to integrate heterogeneous system architectures with specialized units for computing, memory, sensing etc with the stepstone to create new generation of processor designs. However, to maintain an efficient on chip parallel processing among each system on chip (SoC) [], the communication bottleneck had to be solved with scalable interconnections by reducing the additional impairments such as excess power dissipation on wired connections. Network on Chip (NoC) [] introduced a properly structured communication architecture for many core chip packages with a layered design by controlling the traffic congestion on routing network while providing high execution speeds. As the number of cores were started to increase with very large scale SoC integration, the maximum communication latency was not adequate to accommodate the processors. Thus, wireless hybrid networks [] were adopted to cater distant communication links with the compatibility on system in package technologies and cluster based near node architecture was proposed to share data among adjacent nodes. 

Wireless communications at the chip scale, where on-chip antennas establish intra-/inter-chip links using the computing package as propagating medium, have become a promising solution to overcome the profound difficulties demonstrated by current interconnect solutions. This is due to their inherent broadcast capabilities, low latency (even across chips), and flexibility to adapt to varying traffic patterns. In accordance to such promise, several groups have done extensive research on integrated antennas \cite{Pano2020a}, transceivers \cite{yu2014architecture}, protocols \cite{franques2021fuzzy}, and wireless-enabled computer architectures \cite{franques2021widir}. Most works attempt to fulfill the stringent latency ($<$10 nanoseconds), speed ($>$100 Gb/s), and error ($<$10\textsuperscript{-10}) demands of the application with simple and opportunistic solutions, trying to adhere to its stringent energy ($<$1 pJ/bit) and transceiver area ($<$0.1 mm\textsuperscript{2}/Gb/s) limitations. 

%has become a promising solution to overcome the profound difficulties demonstrated on NoC by gaining approximately ten-fold efficiency with proper design and channel characterization. 

However, wave propagation within computing packages produces reverberant energy reflections, hence creating lengthy delay spreads, which in turn hinder high-rate data transmissions with severe Inter-Symbol Interference (ISI) effects. Moreover, high energy spread and correlation due to reverberation prevents the creation of multiple spatial channels concurrently. These aspects have been generally neglected in most prior work in the area \cite{abadal2019wave, timoneda2018channel}, although they are clearly incompatible with the high-speed and resource-efficient vision for wireless communications at the chip scale. 

%degrades the concurrent transmission in same frequency and time due to non-orthogonality. Thus, the signal energy scatters around a confined chip package with a crucial task of demodulating the received data streams at the receivers with low bit error rates (BER), which are to be comply with wired communications. 

%However, the electromagnetic (EM) waves which propagates on chip environment produces reverberant energy reflections, by creating lengthy delay spreads on the receiver cores, which in return hinder high frequency data transmissions with inter symbol interference (ISI). Moreover, high channel correlation due to reverberation degrades the concurrent transmission in same frequency and time due to non-orthogonality. Thus, the signal energy scatters around a confined chip package with a crucial task of demodulating the received data streams at the receivers with low bit error rates (BER), which are to be comply with wired communications. Conventional wireless communication techniques which generate orthogonal precoded wireless beams such as code division multiple access (CDMA) [], orthogonal frequency division multiple access (OFDMA) [] and zero forced beam-forming [] were difficult to be adopted on the chip environment with the complex signal processing and the area/power limitations. Fortunately, as the wireless channels are quasi deterministic with prior characterization and exact channel impulse response can be obtained, the communication can be pre-designed to have the desired EM energy focusing with constructive and destructive interference on the receiver with techniques such as time reversal. 

In this paper, we aim to bridge this gap by jointly addressing the problems of inter-symbol and co-channel interference in reverberant chip packages. To this end, we propose to use Time Reversal (TR) \cite{Han2012, Xu2018, alexandropoulos2022time}. In essence, TR pre-emphasizes the transmitted symbols with the time-reversed version of the channel's response. This creates a spatial matched filter for an intended receiver or, in other words, focuses the signals in time and space around such receiver. \hl{with TR, we demonstrate spatial temporal focusing of EM radiation in a frequency on the lower side of the terahertz spectrum relevant to current efforts in 6G networks and beyond (i.e. 140 GHz).} As shown in Figure~\ref{fig:abstract}, the transmitter targets a specific receiver by choosing the appropriate TR filter. Then, as long as the impulse responses of two different links have a low correlation, multiple concurrent TR transmissions are possible in the same frequency band. This opens the door to the implementation of collective communication patterns that are widespread and extremely relevant in modern computing systems \cite{abadal2016characterization, Karkar2016}.  

\begin{figure}[!t]
\centering
%%\vspace{-0.2cm}
\includegraphics[scale=0.4]{images/system model.pdf}
\vspace{-0.3cm}
\caption{Time reversal for multi-channel wireless communications in a computing package. Through a filter at the transmitter end, time reversal attains spatiotemporal focusing at an intended receiver. If channels are not very highly correlated, multiple concurrent transmissions are possible.}
\label{fig:abstract}
%\vspace{0.4cm}
\end{figure}

While TR and other orthogonal pre-coding alternatives such as CDMA \cite{Vijayakumaran2014}, OFDMA \cite{Hakat2022} and zero-forcing beamforming \cite{Iwabuchi2023} may be difficult to be adopted due to the complexity of the signal processing involved, the particularities of the on-chip scenario allow to simplify these techniques significantly. In our particular case, TR requires knowing the channel response at all times. Fortunately, unlike in conventional scenarios, the wireless in-package channel is static and can be pre-characterized accurately. 

%to go through equivalent reverberant conditions (assuming perfect channel reciprocity) as forward transmission by creating an ideal match filter at the receiver node. With the exact known CIR in WNoC, TR can be easily adopted with minimal signal processing at the transmitter by achieving high spatial temporal focusing in time and space. Moreover, TR naturally compress the interference of concurrent signal transmissions by propagating through lesser correlated channels on adjacent nodes. Therefore, with proper characterized CIR at each core, TR can be adopted to have multiple concurrent signal transmissions with limited interference by sharing same frequency time resources. 

%Conventional wireless communication techniques which generate orthogonal pre-coded wireless beams such as  may be difficult to be adopted on the chip environment due the complex signal processing and the area/power limitations. Fortunately, as the wireless channels are quasi deterministic with prior characterization and exact channel impulse response can be obtained, the communication can be pre-designed to have the desired EM energy focusing with constructive and destructive interference on the receiver with techniques such as time reversal. 

The main contributions of the paper are as follows. We first propose a practical scheme to apply TR for multi-channel wireless chip-scale communications (Figure \ref{fig:abstract}). Then, after providing background on the field in Section \ref{sec:background}, we model different multi-channel TR schemes according to Figure \ref{fig:cases} in Section \ref{sec:model}. We simulate an actual chip package with realistic antennas at 140 GHz and demonstrate that the use of TR allows having multiple simultaneous transmissions that are robust against ISI. We also demonstrate that by taking advantage of symmetric positions in space we can multiplex and use a single terminal to transmit different data frames towards said positions, as described in Section \ref{sec:results}. Finally, we discuss feasibility and possible extensions of the work in Section \ref{sec:discussion} and conclude the paper in Section \ref{sec:conclusion}.

%\hl{The paper explores multiple channels. Cite figure 1}




==> 2-background.tex <==
%\hl{GLOBECOM is a more general conference on communications, and the terahertz symposium is sensitive to new applications, but not necessarily on-chip wireless comms. So here we could provide some background.}
Next, we provide some background about the rationale and concept of Network-on-Chip (NoC) in Section \ref{sec:backNoc}, about the fundamentals of wireless chip-scale communications in Section \ref{sec:backWi}, about the wireless channels within computing packages in Section \ref{sec:backChan}, and about integrated antennas and their placement in Section \ref{sec:backAnt}.

\subsection{Network-on-Chip}
\label{sec:backNoc}
To satisfy the communication needs of multicore chips, Network-on-Chip (NoC) has been the standard interconnect fabric in the last decade \cite{Nychis2012}. NoCs are packet-switched networks of integrated routers and wires typically arranged in a mesh topology. This approach, however, has important limitations when scaled beyond tens of cores. In particular, chip-wide and broadcast transfers suffer from increasing latency and energy consumption due to the many hops needed to reach the destination(s) \cite{Nychis2012}. 

This problem cannot be fixed with longer interconnects due to the dramatic growth in resistivity of copper wires in deeply scaled technology nodes \cite{Todri-Sanial2017}. Further, when moving to multi-chip processors, the concept of NoC has been extended to incorporate off-chip links and form the Network-in-Package (NiP) \cite{Shao2019}, aggravating their existing issues and adding new ones. For instance, NiPs are rigid and prone to over-provisioning. This, together with the connectivity constraints of each chiplet determined by the amount of physical connection pins, severely limits the scalability of the wired approach.

\subsection{Wireless Chip-Scale Communications}
\label{sec:backWi}
%\hl{Rationale of the idea. Why do we need such communications? Comparison with wired. Area and energy constraints lead to high frequencies (to reduce antenna footprint) and simple low-order modulations (to reduce energy consumption as well).}
Wireless communications at the chip scale have been proposed to comply with the particular demands of bandwidth and reconfigurability that NoCs fail to provide. Complementing NoCs with wireless links supplies broadcast support, flexibility in reconfiguration, and low latency by offering wireless paths between distant cores. %Due to this, several groups have devoted efforts in developing hardware and protocols to implement this idea.

%In \cite{abadal2016scalability} the broadcast capabilities of different WNoc schemes are assessed and compared with NoC designs. They considered one antenna per core and a shared channel among all of them. Their results argue that wireless links deliver a latency of an order of magnitude lower than the wired alternative, a trend that is maintained with the increment of cores. They also propose a hybrid approach to take on the benefits of a heterogeneous network in the chip.

%% ARCHITECTURES
% Deja deja :) esto lo hago yo -- las figuras son cruciales, mejor poner tiempo ahí
Several efforts have investigated the impact of having wireless links at the network and system levels. It has been shown that complementing existing wired NoCs/NiPs with wireless channels for broadcast \cite{abadal2016scalability} and long-range links \cite{murray2014performance} can reduce the latency by an order of magnitude and improve throughput significantly, especially when the NoCs and NiPs are scaled. %They also propose a hybrid approach to take on the benefits of a heterogeneous network in the chip.
Further, several studies have investigated impact of having wireless links on the performance of several CPU and accelerator architectures \cite{franques2021widir}, demonstrating that computing can be sped up up to 10$\times$.

%% PROTOCOLS
For the aforementioned impacts to be realized, wireless channels need to be shared among a relatively large number of wireless interfaces. Hence, MAC protocols have been a crucial part of the wireless NoC research, trying to handle variable traffic patterns with very low latency. In this respect, several variants of CSMA \cite{mestres2016mac} and token passing \cite{mansoor2015reconfigurable, franques2021fuzzy} uniquely tailored to the chip-scale environment have been proposed. Also, unconventional approaches such as bit-level contention \cite{duraisamy2015enhancing}, tone-based arbitration \cite{Oh2011}, or reinforcement learning \cite{jog2021one} have been tackled in related work.

%% HARDWARE, TRX
At the physical layer, most wireless NoC proposals have advocated for low-order and simple modulations that avoid power-hungry components. In this respect, On-Off Keying (OOK) prototypes at high frequencies have been presented in multiple works. 
%There are some works that propose transceivers at 60 GHz with simple modulations to minimize area and power consumption \cite{yu2014architecture}. 
In \cite{yu2014architecture}, a direct OOK modulator and non-coherent receiver is implemented with 65-nm CMOS, achieving 16 Gb/s with a central frequency of 60 GHz. The authors discuss how this could be extended to a triple-channel scheme achieving 48 Gb/s with 2 pJ/bit at an error rate below 10\textsuperscript{-12} and taking 0.75 mm\textsuperscript{2} of chip area. In \cite{Holloway2021,Yi2021}, the authors discuss how such designs could be taken to 300 GHz with SiGe and InP technology as well.
%Simple modulations such as on-off keying Impulse radio and continuous wave, amplitude shift keying (ASK), pulse position modulation (PPM) and binary phase shift keying (BPSK) can be exploited and adopted to wireless data communication to transmit more symbols in the same bandwidth and it was proved that ASK with 16dB AWGN can provide a BER of $10^{-15}$ in 10Gb/s, which comply with the stringent BER requirement of wired communication.


\subsection{Wireless Channels within Packages}
\label{sec:backChan}
%\hl{Summary of types of packages and the type of channel that you can have. Mention that some of the enclosed packages can lead to reverberation, and hence to ISI if we want fast rates.}
Typically a chip consists of a lossy silicon substrate with several layers of metal stack on top and separated by dielectric layers \cite{markish2015chip}. There are several ways of connecting a chip with the rest of the system and enclosing it within the package. A commonly used package in modern computing systems is the flip-chip. There are several variants of it, depending on whether 2D, 2.5D, or 3D integration is considered. The classical 2D variant has, from the PCB up, a layer of solder bumps, followed by a thin layer of dielectric insulator, where the interconnects are, with the silicon substrate and the heat sink on top \cite{wright2006characterization}.  
% Because we are working in a processor environment our implementation would take place in a fully enclosed chip. 
%Flip chips are popular because of their lower inductance and higher power/bandwidth density. 
In the 3D variant of a flip-chip package, several chips are stacked and interconnected by means of Through-Silicon Vias (TSV). Finally, to interconnect multiple chips in a 2.5D fashion, chips are placed side-to-side on top of a silicon interposer via an array of micro-bumps. The interposer is connected to the PCB through the solder bumps \cite{zhang2015heterogeneous}. For the sake of generality, the work developed in this paper takes place in an interposer package. 

%Wirebonding packages are popular in low-power processor architectures. As opposed to the flip chip, the chip is mounted directly on the substrate and connected to the  circuitry by wires. 

%Although some works propose a packageless approach and open die configurations \cite{pal2018case}.

As in large-scale wireless environments, the electromagnetic wave propagating in the chip will be affected by reflections, refractions, diffractions, and absorption phenomena \cite{chen2019channel}. This is paired with the fact that the system desired for our application takes place in an enclosed environment, therefore the package can be seen as a reverberation chamber \cite{Matolak2013CHANNEL}. All the energy propagating around the structure produces a multipath-rich environment that creates notches in the frequency response and lengthens the channel in time. The actual length of the channel depends mostly on the dimensions and resistivity of the silicon layer, which is a major contributor on the channel losses \cite{imani2021smart}. In any case, as we increase the symbol rate to meet the BER conditions, the delay spread of the channel leads to ISI which undermines further the quality of transmission \cite{Rayess2017}. 


\subsection{Integrated Antennas}
\label{sec:backAnt}
%\hl{Summary of where you can integrate antennas, type that you can have. Change this is still not done}
%On-chip antennas are the cornerstone of wireless chip-scale communications and their design and placement are crucial. 
The placement of an antenna within a computing package is complex as it is a densely integrated environment. In general, there are two strategies that we refer to on-chip integration and in-package integration. Several alternatives have been implemented across the spectrum, from millimeter-wave to optics, using both strategies \cite{abadal2019wave}. 

%% FULL INTEGRATION (horizontal)
%% FULL INTEGRATION (vertical, TSV antennas)
On the one hand, on-chip antennas can be horizontally or vertically co-integrated with the transceiver circuits. Horizontal designs generally use the metallization layers of a chip \cite{branch2005wireless} to implement variants of a dipole (meander, zig-zag), bow-tie or Yagi-Uda antenna \cite{guo2002propagation, gutierrez2009chip, Rayess2017, bellanca2017integrated, narde2018chip}. Here, the main decision is whether to use the layers closer to the silicon layer or closer to the bumps. The former leads to very low gains due to the impact of lossy silicon, whereas the latter is impractical as the proximity to the bumps will short-circuit the antenna. %\hl{merge} 
%To place the antennas horizontally could be a solution to enable larger wires and therefore not such a demanding operation frequency. However, placing many horizontal wires in this approach could lead to a waste of space not affordable in the chip. There are some works that propose printed antennas instead of wire, and propose planar structures like patches, meander or folded dipoles \cite{guo2002propagation, gutierrez2009chip, Rayess2017}. The shortcoming of using planar structures is that we relinquish an omnidirectional radiation pattern, which is desirable for the wave propagation to get to their neighbor antenna.

%Placing the antennas far from the silicon as some works proposed is unrealistic since locating the antennas in the metal layers leads to impaired transmission because the metal bumps obstruct the channel path \cite{branch2005wireless}. Also, an antenna placed in proximity to the bumps will become short-circuited by the metal. The location of printed dipoles or patches in the metal layers close to the silicon has been proposed \cite{timoneda2018channel}, however, the efficiency of the antenna is once again compromised by the metal plane. 

The alternative to the horizontal approach is the implementation of antennas via a vertical approach, as in \cite{timoneda2018channel,Pano2020a,wu2017monopoles}, where the authors propose to use TSVs as vertical monopoles. This allows for the radiation to happen laterally towards other antennas this is paired with the use of image theory, with the metal layer acting as ground plane so the monopole can be considered as a dipole. Although vertical antennas only support high frequencies due to the relatively small lengths of typical TSVs, in this paper we follow this approach due to its superior co-planar coupling and reduced area footprint.
%A possible issue of this approach is the height restriction regarding the package, of only a few mm. So for the antennas to fit vertically in the chip, very high resonant frequencies are imposed to meet the miniaturization requirement. This approach is followed by us in this work. 

%% IN-PACKAGE INTEGRATION 
On the other hand, in-package integration refers to the stacking of an antenna module (with its own ground plane and substrate) on top of the chip and the interconnection of the on-chip transceiver and the in-package antenna with a TSV. This allows to electromagnetically isolate the antenna from the layers underneath, reducing losses and allowing for a wider range of antenna designs, at the cost of adding manufacturing steps, cost, and reverberation \cite{hwangbo2019integrated,yeh2012design}. %\hl{merge} Some work has been developed to design antennas that comply with having compact features and providing large bandwidths to support the increasing data rates of multi-core systems, such as meander dipole, zigzag dipole, slot, loop, inverted F, bow-tie and Yagi \cite{hwangbo2019integrated,yeh2012design,wu2017monopoles,bellanca2017integrated, hahnel2015integrated, narde2018chip}.


%The integration of one or more antennas per core means a reduction in its area. To achieve an antenna that fits in the constraint space and that occupies minimal chip space implies structures working at very high frequencies \cite{Rayess2017, wu2017monopoles, timoneda2018modeling}, which also provide larger bandwidths.

%The recent advancements in radio frequency (RF) technology, miniature antenna and transceiver designs from millimeter (mm) wave–terahertz (THz) frequency bands have been studied and evaluated with 16nm CMOS integration. Few experimental research studies have been demonstrated that these antennas provide an acceptable power gain and area overhead in related to wireless on chip applications. WNoC limits the IC overheads and additional impairments such are area and power with limited wired connections, direct communication links to distinct cores and static transceiver designs which can be reused. 



%\begin{figure}[!t]
%\centering
%%\vspace{-0.2cm}
%\includegraphics[width=0.7\columnwidth]{example-image}
%\vspace{-0.4cm}
%\caption{\hl{Figure showing the chiplet-based interposer environment, also showing the position of the antennas you use in the simulations (give it names: A, B, C, D), and perhaps an inset with the antennas you assumed in the simulations.}}
%\label{fig:environment}
%\vspace{0.4cm}
%\end{figure}



==> 4-results.tex <==



%\hl{vert briefly explain the workflow: you obtain the CIR of multiple channels with CST full-wave simulation, this is imported in matlab, where it is time reversed. Then multiple transmissions are simulated using the system model presented before. Consider adding a table with some parameters: frequency, dimensions, modulation, number of TX-RX, etc...}
To evaluate the proposed approach, we first simulate the chip environment using CST Microwave Studio \cite{CST}. We build a realistic model of an interposer package described in Sec.~\ref{sec:backChan} with twelve antennas in four chiplets (Fig. \ref{fig:cases}). Chiplets are 5$\times$5 mm\textsuperscript{2} with 0.5-mm high-resistivity (HR) silicon and 0.5-mm aluminum nitride as heat spreader, on top of a 0.1-mm HR silicon interposer. We obtain the CIR by means of the full-wave solver, to then perform TR simulations in MATLAB. Our aim is to assess the possibility of having concurrent transmissions with distinct TX-RX pairs (Sec. \ref{mtr}) and from one TX to multiple RX (Sec. \ref{mrx}).
%. In the scatter case we want to prove that we are able to have transmission of multiple and different messages from one antenna towards different terminals. 
%Following the methodology described above, we excite Node A (see Figure \ref{fig:cases}) with the corresponding time reversed channel between A and B, simultaneously we do the same for the link E to F and link C to D.     

%In our other case under study 
% fatima, explica el detalle de los use cases en cada subseccion. es decir, empieza IV-B diciendo que los links considerados son AB, con CD y EF como interferentes; en IV-C dices que A transmite para X, Y, Z simultaneamente.




\subsection{Wireless Channel}
Figure \ref{fig:channel} summarizes the simulations made to illustrate how TR works in an interposer package with vertical monopoles operating at 140 GHz. Fig.~\ref{fig:channel}(a) shows how the antennas resonate at $\sim$138 GHz. The power received across the 135--145 GHz band shows notches, suggesting the presence of strong multipath. Panels \ref{fig:channel}(b) and \ref{fig:channel}(c) demonstrate the spatiotemporal focusing effect of TR by plotting the spatial and temporal field distribution, respectively. Spatially, we observe the non-TR transmission being scattered across the four chiplets, while the TR case is clean and only focuses the energy around very specific spots. In time, we observe a strong peak in the TR response at the intended receiver, much higher than the level of non-TR transmission. Finally, Fig.~\ref{fig:channel}(d) shows how TR compresses the interference to non-targeted receivers, as long as their channel is not correlated with the intended one. Here, this is the case of node $C$, which is located in a close-to-symmetric position to $B$ with respect to $A$.

%\hl{Fatima's simulations of the antenna (S11) and channel (S21). Comparison of TR vs non-TR in terms of field distribution and temporal shape of the response, Maybe also compare the power in intended and non-intended positions.}

%To evaluate the spatial selectivity of the TR technique in the interposer package, we also obtain the energy $E(i,j,k)$ received in node $k$ when node $i$ transmits with TR towards node $j$,
%\begin{equation}
%    E(i,j,k) = \int{h_{ik}(t) * h_{ij(-t)}} \partial t.
%\end{equation}


\subsection{Multiple Transmitters}\label{mtr}
%\hl{Show that we can have multiple transmissions at the same time.} 
Following the methodology described in Section \ref{sec:results}, we excite Node A (see Figure \ref{fig:cases}) with the corresponding time reversed channel between A and B, and simultaneously we do the same for the link E to F and link C to D. To evaluate the capacity of TR to support multiple channels, we obtain the SINR at each core based on the received signals as mentioned in Section \ref{multlink}. 

%Let us consider the signal and the interference focused at node $i$ as $y_{ij}$ and $y_{I}$ respectively. 

%\begin{equation}
%\begin{split}
%    y_{ij}& = h_{ij}(t) * h_{ij}(-t) * m_{i}(t)+n_{j}(t) \\
%    y_{I} &= \sum_{l\in L,l\neq i} h_{lj}(t) * h_{l}(-t) * m_{l}(t)+n_{j}(t)\\ 
%\end{split}    
%\end{equation}

% fatima creo que qutaremos esta formulacion

%Therefore, the SINR for $L$ TR links can be obtained with the instantaneous energy detection at node $j$  as below.
%\begin{equation}
    %SINR_{j} = \frac{\sum_{k_1} |y_{ij}|^2 }{\sum_{k_2} |y_{I}|^2+n_{j}(t)}
%\end{equation}
%where $k_1$ and $k_2$ are the convoluted multi-path components of the focused EM distribution at node $j$. Note that each CIR is normalized with the square root of its power. 

%Figure \ref{fig:multi-link} \hl{Ama please explain - merge with below}

The performance of multi-link TR transmissions were analysed in terms of SINR and BER with 140GHz center frequency. With promising results demonstrated by ASK with single TR link, the ASK modulated bit stream with 140GHz carrier was sent through TR filter as mentioned in Section \ref{multlink} and demodulated with respective thresholds for \{0,1\}. The performance measurements were obtained with respect to three cases; case (I) single link TR transmission ; case (II) two parallel link TR transmission; case (III) three parallel link TR transmission.
The SINR measurements were obtained with respect to the transmitted power from -5dBm to 10dBm and case (I) results were compared with a non-TR signal transmission. In Figure \ref{fig:multi-linka}, it was observed a 8dB SINR gap between TR and non-TR transmissions, which shows that TR improves the received signal by minimising the interference. Moreover, when the amount of parallel transmissions were increased the SINR was reduced consequently with the increment of co-channel interference. The case (II) performance was further analysed with two different channels and it was observed that based on channel correlation the interference compression of TR filtered signals can be differed from one channel to another.\par
The performance in terms of BER was also analysed in terms of aforementioned three cases. The Figure \ref{fig:multi-linkb} demonstrates the BER performance with respect to the gradual increment of transmitted power for each node. The analysis was conducted from 0dBm to 13dBm to measure the impact of co-channel interference, as with the  increment of power the received signal strength increases and consequently the interference increases. The simulations were conducted for 50Gb/s fixed data rate and -13.9dB AWGN noise. It was observed for single TR link BER saturates approximately around 11.7dBm and while for three parallel transmissions, the BER starts to increase around 8.45dBm. Two parallel links perform in a similar manner though the BER values can be varied with the received signal strength of each channel in relative to the channel correlation. Note that the power is equally distributed among each transmitted bit. \par 
In Figure \ref{fig:multi-linkc} the BER was measured with data rate with a fixed transmission power of 10dBm. It was demonstrated that with gradual increment in the dta rate the BER also increases and when the nuber of parallel transmissions are increased with equal power, the impact of interference is increased and BER is saturated with limited rates. 


%(b) for all the cases mentioned above (here we should see how at low Ptx, noise dominates and BER goes down when Ptx increases, up to a point where interference dominates and increasing Ptx does no longer reduce BER -- and that this point is worse when we have more interferers)
% for all the cases mentioned above (we should see something similar than in the other figure; first noise doiminats and then interference dominates)


\begin{figure*}[!t]
\centering
%%\vspace{-0.2cm}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\textwidth]{images/sinr1.eps}
\caption{}
\label{fig:multi-linka}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BER1fixeddata.eps}
\caption{}
\label{fig:multi-linkb}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BER11fixedpower.eps}
\caption{}
\label{fig:multi-linkc}
\end{subfigure}
\vspace{-0.2cm}
\caption{Time reversal with multiple concurrent transmitters. (a) 
SINR for non-TR and TR cases with single or multiple links and increasing the transmitted power. (b) BER as a function of transmitted power for a data rate of 50 Gb/s for an increasing number of links. (c) BER as a function of the aggregated data rate for a power of 10 dBm per transmitter.}
\label{fig:multi-link}
\end{figure*}

\subsection{Multiple Receivers} \label{mrx}
%Show that we can have multiple messages from a single transmitter to multiple receivers at the same time.
Next, we show the results of transmitting from $A$ to $C$-$D$. We remind that $A$ sends different chunks of data to each receiver thanks to TR multiple access as described in \cite{Han2012}. \par


%Figure \ref{fig:scatter} \hl{Ama please explain}

As similar to Section \ref{mtr}, the SINR and BER was analysed in receiver B, with the impact of co-channel interference on concurrent transmissions. It was observed in Figure \ref{fig:scattera}, the SINR for multiple transmissions have been decreased in compared to the measurements in Figure \ref{fig:multi-linka}, as in single transmitter multiple TR links are active to perform concurrent transmissions. With the effect of multi-path components of CIR in superimposed channels, the focused EM distribution could reduce the received signal strength with a minor amount, while maintaining the interference suppression.\par 
In Figure \ref{fig:scatterb}, the BER performance was measured with a fixed data rate of 50Gb/s, with increased power values upto 10dBm. It was observed that as the transmitter power increases gradually the impact of interference increases and as the correlation of  channel A to D and A to B is higher in compared with A to C, the BER is increased with high interference. The channel correlation has similarly affected three concurrent transmissions by increasing the BER while demonstrating an early BER saturation with transmit power. \par 
The BER measurements in Figure \ref{fig:scatterc}, shows the effect of interference on parallel receivers for 10dBm transmit power with increased data rate. A similar BER performance with increased interference is observed in compared with Figure \ref{fig:multi-linkc}, while the BER take higher
values with minor increment based on superimposed TR transmissions. \par 


\begin{figure*}[!t]
\centering
%%\vspace{-0.2cm}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\textwidth]{images/sinr2.eps}
\caption{}
\label{fig:scattera}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BER2fixeddata.eps}
\caption{}
\label{fig:scatterb}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[width=\textwidth]{images/BER2fixedpower.eps}
\caption{}
\label{fig:scatterc}
\end{subfigure}
\vspace{-0.2cm}
\caption{Time reversal with multiple concurrent receivers. (a) 
SINR for non-TR and TR cases with single or multipe receivers and increasing the transmitted power. (b) BER as a function of transmitted power for a data rate of 50 Gb/s for an increasing number of receivers. (c) BER as a function of the aggregated data rate for a total power of 10 dBm.}
%\caption{\hl{(a) SINR for receiver B when A transmits, in different cases (alone, when we also want to transmit to two receivers, B and C, B and D, and B-C-D) as a function of the transmitted power, (b) BER as a function of transmitted power, fixing data rate, for all the cases mentioned above (we should see something similar than in the other figure; first noise doiminats and then interference dominates) (c) BER as a function of the TOTAL data rate, fixing transmitted power, for all the cases mentioned above.}}
\label{fig:scatter}
%\vspace{0.4cm}
\end{figure*}



==> 5-discussion.tex <==
%\hl{Fatima: discuss how due to symmetries, there could be multiple potential points receiving the same; and this could be combined with the multi-link example. Point to figure 3 which has two symmetric peaks and the impact of close-to-symmetric positions. If time allows, show two groups of symmetric peaks, this is, combining the results of the paper with a careful choce of symmetric points. Also talk about the need of perfect filters to harness the power of TR, and that we plan to investigate how TR degrades with simpler filters.}

TR can be used to achieve a perfect concentration of energy in time and space in point to point links and simultaneously compress the interferences that might affect the transmission. If we consider a scenario with many antennas carefully placed, we can use symmetries to have multiple positions where the terminals will obtain the same response.
To explain this further, let us refer to Figure \ref{fig:channel}(b), where we see two peaks of highly concentrated field. These peaks are obtained at unison with a single excitation of the transmitter because they are placed in a symmetric location that makes their channel responses identical. These links will have equal concentration in space and compression in time. This is beneficial to us because we can have multicast transmissions using one CIR.

As for the rest of the links in the landscape, the effects of TR become larger as the terminals get close to the symmetry point of the corresponding CIR. In Figure\ref{fig:channel}(d) we can see a perfect example of this. So the highest energy concentration happens in node B because it's CIR is the one we use to compensate the channel during transmissions. In nodes D, E, and F the concentration is negligible because these nodes are not in symmetry points and therefore these links channels cant be compensated by node B CIR. However, in node C there is a rise in power concentration. This is due to node C being close to the point where the CIR becomes correlated and similar to that of node B.

TR technique can be viewed as a sort of perfect filter to heighten the signal reception and transmission while suppressing unwanted interference. Yet, a perfect filter for real world applications is somewhat unrealistic. We aim to explore the trade-off, limitations, and performance degradation that arise with the use of non-ideal filters. 





==> 6-conclusion.tex <==
In this paper we have conducted simulations in a multicore package in the terahertz band to explore the effects of TR in transmission performance. We can take advantage of the knowledge we have on our architecture to get the correct and invariant CIR of the wireless paths and use them to create many channels in space.

More than staying in a single point to point link, in this paper we wanted to test the possibility of multiple concurrent and independent transmitters, and also the other way around with several simultaneous receivers.The TR capabilities were tested by obtaining the SINR with respect to the transmitted power, the BER vs the transmission power and BER vs Data rate.

Comparing the SINR of TR and non-TR transmissions we have a heightened signal that shows TR improvement. With the increment of simultaneous wireless links, we got a decrement in SINR due to the correlation between links in positions close to symmetry. Similarly, when we increase the number of antennas receiving from a single sender, the SINR starts to decrease because there is a limit on the amount of CIR you can superimpose in a single transmission. We could check that the BER saturates faster with the increment of parallel transmitters and receivers. For transmission power up to 8 dBm the BER remains in good values. We have shown we can have parallel terminals transmitting in unison and multicast transmission in one-to-many fashion. All of these can be attained in the same frequency thanks to  the interference compression of TR.
